AI Agents Under Threat: A Survey of Key Security Challenges and Future Pathways

An Artificial Intelligence (AI) agent is a software entity that autonomously performs tasks or makes decisions based on pre-defined objectives and data inputs. AI agents, capable of perceiving user inputs, reasoning and planning tasks, and executing actions, have seen remarkable advancements in algorithm development and task performance. However, the security challenges they pose remain under-explored and unresolved. This survey delves into the emerging security threats faced by AI agents, categorizing them into four critical knowledge gaps: unpredictability of multi-step user inputs, complexity in internal executions, variability of operational environments, and interactions with untrusted external entities. By systematically reviewing these threats, this paper highlights both the progress made and the existing limitations in safeguarding AI agents. The insights provided aim to inspire further research into addressing the security threats associated with AI agents, thereby fostering the development of more robust and secure AI agent applications.

==> figures/Main_Agent_mindmap.tex <==
% \begin{figure*}[!ht]
% \scriptsize
%     \begin{adjustbox}{width=\textwidth}
%         \begin{forest}
%         for tree={
%                 forked edges,
%                 grow'=0,
%                 draw,
%                 rounded corners,
%                 node options={align=center},
%                 text width=2.7cm,
%                 s sep=6pt,
%                 calign=edge midpoint, 
%             },
%                 [Main Agent Security, fill=gray!45, parent
%                     [Prompt template Risk \S\ref{sec:mainagent:prompt} , for tree={action} 
%                     [\hphantom{x} Jailbrek 
%                             [{},action_work]
%                             [{}, action_work]
%                         ]
%                     [Prompt Injection\cite{liu2023prompt}
%                             [{prompt  injection attacks\cite{perez2211ignore}}, action_work]
%                             [{black prompt injection attacks\cite{liu2024prompt} }, action_work]
%                             [{indirect prompt injection\cite{greshake2023youve}}, action_work]
%                         ]
                   
%                     ]
                    
%                     [LLM-based Risk
%                     \S\ref{sec:mainagent:llm}, action
%                         [Privacy Risk
%                             [{Multi-Step Jailbreaking Prompts (MJP) to extract (name, address) pairs \cite{li2023multi}}, action_work]

%                              [{LLMs to re-identify personal information\cite{nyffenegger2023anonymity}}, action_work]
%                         ]
%                         [Unsafe code execution
%                             [{Maliciously executing unsafe code: SOL injection\cite{pedro2308prompt}, RCE\cite{liu2023demystifying}}, action_work]
%                             [{ Instructions Underspecification Risk\cite{ruan2023identifying}},action_work]
%                         ]
%                           [Cyber Theat Assitant
%                             [{}, action_work]
%                           ]
%                           [Agent Society Risk
%                             [{}, action_work]
%                         ]
%                     ]

%                 [Reasoning Risk
%                     \S\ref{sec:mainagent:reason}, 
%                     action
%                     [Haullunation
%                             [{}, action_work]
%                           ]
%                     [Alignment
%                             [{}, action_work]
%                     ]
%                     [Generalize
%                             [{Enhance generalization with training dataset \cite{li2023api, liu2023agentbench, qin2023toolllm,huang2023metatool}}, action_work]
                            
%                             [{Enhance generalization with RL \cite{}}, action_work]
                             
%                     ]
                       
%                 ]
%             ]
            
%         \end{forest}
%     \end{adjustbox} 
%     \caption{Typology of the Main Agent risk module.}
%     \label{fig:sec5_mindmap_action}
% \end{figure*}
% \begin{figure*}[!ht]
% \scriptsize
%     \begin{adjustbox}{width=\textwidth}
%         \begin{forest}
%         for tree={
%                 forked edges,
%                 grow'=0,
%                 draw,
%                 rounded corners,
%                 node options={align=center},
%                 text width=2.7cm,
%                 s sep=6pt,
%                 calign=edge midpoint, 
%             },
%             [Main Agent Security, fill=gray!45
%                 [Prompt Template Risk \S\ref{sec:mainagent:prompt}, for tree={fill=gray!30}
%                     [Jailbreak
%                         [Placeholder for Action, edge label={node[midway,fill=white]{Detail}}]
%                         [Placeholder for Action]
%                     ]
%                     [Prompt Injection \cite{liu2023prompt}
%                         [Prompt Injection Attacks \cite{perez2211ignore}]
%                         [Black Prompt Injection Attacks \cite{liu2024prompt}]
%                         [Indirect Prompt Injection \cite{greshake2023youve}]
%                     ]
%                 ]
%                 [LLM-based Risk \S\ref{sec:mainagent:llm}, for tree={fill=gray!30}
%                     [Privacy Risk
%                         [Multi-Step Jailbreaking Prompts to Extract (Name, Address) Pairs \cite{li2023multi}]
%                         [Using LLMs to Re-identify Personal Information \cite{nyffenegger2023anonymity}]
%                     ]
%                     [Unsafe Code Execution
%                         [Maliciously Executing Unsafe Code: SOL Injection \cite{pedro2308prompt}, RCE \cite{liu2023demystifying}]
%                         [Instructions Underspecification Risk \cite{ruan2023identifying}]
%                     ]
%                     [Cyber Threat Assistance
%                         [Placeholder for Action]
%                     ]
%                     [Agent Society Risk
%                         [Placeholder for Action]
%                     ]
%                 ]
%                 [Reasoning Risk \S\ref{sec:mainagent:reason}, for tree={fill=gray!20}
%                     [Hallucination
%                         [Placeholder for Action]
%                     ]
%                     [Alignment
%                         [Placeholder for Action]
%                     ]
%                     [Generalization
%                         [Enhance Generalization with Training Dataset \cite{li2023api, liu2023agentbench, qin2023toolllm,huang2023metatool}]
%                         [Enhance Generalization with Reinforcement Learning \cite{}]
%                     ]
%                 ]
%             ]
%         \end{forest}
%     \end{adjustbox} 
%     \caption{Typology of the Main Agent risk module.}
%     \label{fig:sec5_mindmap_action}
% \end{figure*}



jk
% \begin{figure*}[!ht]
% \scriptsize
%     \begin{adjustbox}{width=\textwidth}
%         \begin{forest}
%         for tree={
%                 forked edges,
%                 grow'=0,
%                 draw,
%                 rounded corners,
%                 node options={align=center},
%                 text width=2.7cm,
%                 s sep=6pt,
%                 calign=edge midpoint, 
%             },
%                 [  User Security \S\ref{sec:usersecurity}, fill=gray!45, parent
%                     [User input risk \S\ref{sec:usersecurity:userinput} , for tree={action} 
%                         [\hphantom{x} Human feedback risk \S\ref{sec:usersecurity:userinput:human}
%                             [{},action_work]
%                             [{}, action_work]
%                         ]
%                          [\hphantom{x} User introction underspecification risk\S\ref{sec:usersecurity:userinput:userinstruction}
%                             [{},action_work]
%                             [{}, action_work]
%                         ]
%                     ]

%                     [Malicious user risk \S\ref{sec:usersecurity:malicious} , for tree={action} 
%                           [\hphantom{x} Maliciously executing unsafe code risk \S\ref{sec:usersecurity:malicious:unsafe code} 
%                             [{REC\cite{liu2023demystifying}},action_work]
%                             [{SQL injection\cite{pedro2308prompt}}, action_work]
%                         ]

%                          [LLM agent abuse risk \S\ref{sec:usersecurity:malicious:llm}
%                               [{Generating malicious content,phishing emails\cite{karanjai2022targeted},false information\cite{de2023chatgpt}},action_work]
                            
%                             [{Social engineering attack,phishing websites\cite{roy2023chatbots},malware
%                             \cite{gupta2023chatgpt}}, action_work]

%                             [{Amplification of model biases}, action_work]
%                         ]

%                           [\hphantom{x} Jailbrek risk \S\ref{sec:usersecurity:malicious:jailbreak}
%                             [{},action_work]
%                             [{}, action_work]
%                         ]
                        
%                         [Prompt Injection\cite{liu2023prompt}
%                             [{prompt  injection attacks\cite{perez2211ignore}}, action_work]
%                             [{black prompt injection attacks\cite{liu2024prompt} }, action_work]
%                             [{indirect prompt injection\cite{greshake2023youve}}, action_work]
%                         ]
%                     ]
%             ]        
%         \end{forest}
%     \end{adjustbox} 
%     \caption{Typology of the environment risk module.}
%     \label{fig:sec3_mindmap_action}
% \end{figure*}


\begin{figure*}[!ht]
\scriptsize
    \begin{adjustbox}{width=\textwidth}
        \begin{forest}
        for tree={
                forked edges,
                grow'=0,
                draw,
                rounded corners,
                node options={align=center},
                text width=2.7cm,
                s sep=6pt,
                calign=edge midpoint, 
            },
                [Personal Agent Security, fill=gray!45
                    [Prompt Template Risk 
                    \S\ref{sec:mainagent:prompt},
                    for tree={fill=gray!30}
                        [Adversarial Prompt Risk \S\ref{sec:mainagent:prompt:adver}
                            [Detailed description needed here]
                            [Another detailed description needed here]
                        ]
                        
                        [Trigger Injection Risk \S\ref{sec:mainagent:prompt:trigger}
                            [Adversarial Trigger Injection Risk
]
                            [Backdoor Trigger Injection Risk]
                        ]
                     
                    ]
                    
                    [LLM-based Risk\S\ref{sec:mainagent:llm}, for tree={fill=gray!20}
                        [Privacy Risk \S\ref{sec:mainagent:llm:privacy}
                               [Detailed description needed here]
                            [Another detailed description needed here]
                        ]

                          [Vector Database Text Embedding Risk \S\ref{sec:mainagent:llm:text}
                               [Detailed description needed here]
                            [Another detailed description needed here]
                        ]

                        [LLMs Inversion Risk \S\ref{sec:mainagent:llm:inversion}
                               [Detailed description needed here]
                            [Another detailed description needed here]
                        ]

                            [Unsafe Training Data Risk \S\ref{sec:mainagent:llm:insecure}
                               [Detailed description needed here]
                            [Another detailed description needed here]
                        ]

                        [LLMs Cognitive Risk \S\ref{sec:mainagent:llm:cognitive}
                               [Detailed description needed here]
                            [Another detailed description needed here]
                        ]

                      ] 

                       [Reasoning Risk \S\ref{sec:mainagent:reason}, for tree={fill=gray!30}
                        [Generalization risk  \S\ref{sec:mainagent:reason:gener}
                            [Detailed description needed here]
                            [Another detailed description needed here]
                        ]
                        
                        [Misalignment Risk \S\ref{sec:mainagent:reason:haullucination}
                             [Detailed description needed here]
                            [Another detailed description needed here]
                        ]

                          [Hallucination Risk \S\ref{sec:mainagent:reason:misalign}
                             [Detailed description needed here]
                        ]
                   
                    ]
                ]
                
        \end{forest}
    \end{adjustbox} 
    \caption{Typology of the main agent risk module.}
    \label{fig:sec3_mindmap_env}
\end{figure*}


==> figures/env_mindmap.tex <==
% \begin{figure*}[!ht]
% \scriptsize
%     \begin{adjustbox}{width=\textwidth}
%         \begin{forest}
%         for tree={
%                 forked edges,
%                 grow'=0,
%                 draw,
%                 rounded corners,
%                 node options={align=center},
%                 text width=2.7cm,
%                 s sep=6pt,
%                 calign=edge midpoint, 
%             },
%                 [Environment Security , fill=gray!45, parent
%                     [Virtual Environment \S\ref{sec:envsecurity:vir} , for tree={action} 
%                     [\hphantom{x} Simulated \& Sandbox Environment, action
%                             [{Anthropomorphic Attachment Risk for users~\cite{park2023generative}}, action_work]
%                             [{Simulated Misinformation and Persuasion Vulnerability~\cite{pan2023risk}}, action_work]
%                         ]
%                     [Development \& Testing Environment, action
%                             [{Data breach Risk}, action_work]
%                             [{Unauthorized Access Risk}, action_work]
%                             [{Model Manipulation Risk}, action_work]
%                         ]
%                     [Computing Resources Management Environment, action
%                             [{Inefficient Resource Allocation Risk~\cite{huenabling}}, action_work]
%                             [{Insufficient Isolation Between Agents Risk~\cite{soice2023can,andreas2022language,liang2023encouraging}}, action_work]
%                             [{Unmonitored Resource Usage Risk on LLM agent~\cite{andreas2022language}}, action_work]
%                         ]
%                     ]
                    
%                     [Physical Environment \S\ref{physical_env}, action
%                         [\hphantom{x} Risk of Sensory Integration and Processing, action
%                             [{Hardware Information Leakage Risk～\cite{mrabet2020survey}}, action_work]
%                             [{Outdated Hardware Source Risk～\cite{}}, action_work]
%                             [{Agent System Information Integrity Risk～\cite{}}, action_work]
%                         ]
%                         [Risk of Dynamic Movement and Control , action
%                             [{Hardware Execution Error~\cite{}}, action_work]
%                             [{Low Tolerance Risk in Physical Environment~\cite{}}, action_work]
%                         ]
%                     ]
%                 ]
%         \end{forest}
%     \end{adjustbox} 
%     \caption{Typology of the environment risk module.}
%     \label{fig:sec3_mindmap_action}
% \end{figure*}
\begin{figure*}[!ht]
\scriptsize
    \begin{adjustbox}{width=\textwidth}
        \begin{forest}
        for tree={
                forked edges,
                grow'=0,
                draw,
                rounded corners,
                node options={align=center},
                text width=2.7cm,
                s sep=6pt,
                calign=edge midpoint, 
            },
                [Environment Security, fill=gray!45
                    [Virtual Environment \S\ref{sec:envsecurity:vir}, for tree={fill=gray!30}
                        [Simulated \& Sandbox Environment
                            [Anthropomorphic Attachment Risk for users~\cite{park2023generative}]
                            [Simulated Misinformation and Persuasion Vulnerability~\cite{pan2023risk}]
                        ]
                        [Development \& Testing Environment
                            [Data breach Risk]
                            [Unauthorized Access Risk]
                            [Model Manipulation Risk]
                        ]
                        [Computing Resources Management Environment
                            [Inefficient Resource Allocation Risk~\cite{huenabling}]
                            [Insufficient Isolation Between Agents Risk~\cite{soice2023can,andreas2022language,liang2023encouraging}]
                            [Unmonitored Resource Usage Risk on LLM agent~\cite{andreas2022language}]
                        ]
                    ]
                    [Physical Environment \S\ref{physical_env}, for tree={fill=gray!20}
                        [Risk of Sensory Integration and Processing
                            [Hardware Information Leakage Risk~\cite{mrabet2020survey}]
                            [Outdated Hardware Source Risk]
                            [Agent System Information Integrity Risk]
                        ]
                        [Risk of Dynamic Movement and Control 
                            [Hardware Execution Error]
                            [Low Tolerance Risk in Physical Environment]
                        ]
                    ]
                ]
        \end{forest}
    \end{adjustbox} 
    \caption{Typology of the environment risk module.}
    \label{fig:sec3_mindmap_env}
\end{figure*}


==> figures/interaction_mindmap.tex <==
% \begin{figure*}[!ht]
% \scriptsize
%     \begin{adjustbox}{width=\textwidth}
%         \begin{forest}
%         for tree={
%                 forked edges,
%                 grow'=0,
%                 draw,
%                 rounded corners,
%                 node options={align=center},
%                 text width=2.7cm,
%                 s sep=6pt,
%                 calign=edge midpoint, 
%             },
%                 [Interaction Security , fill=gray!45, parent
%                     [Memory Interaction Risks \S\ref{memory_interaction} , for tree={action} 
%                     [\hphantom{x} Short-term Memory Interaction Risks, action
%                             [In-context Window Limitation Risks, action_work]
%                             [Membership Inference Attack Risks~\cite{wen2023last,duan2023privacy}, action_work]
%                         ]
%                     [\hphantom{x} Long-term Memory Interaction Risks, action
%                             [{Poisioning Attack Risks by Indexing Processing~\cite{zou2024poisonedrag,cohen2024here}}, action_work]
%                             [{Extracting Private Datasets Risks~\cite{zeng2024good} }, action_work]
%                             [{RAG Generation Risks~\cite{kang2024c,hatalis2023memory}}, action_work]
%                         ]
%                     ]
                    
%                     [API \& Tool Interaction Risks \S\ref{tool_interaction}, action
%                         [\hphantom{x} API Use Risks, action
%                             [Authorization Risks\cite{google+, facebook}, action_work]
%                         ]
%                         [\hphantom{x} API Intrinsic Risks, action
%                             [API Security Flaws, action_work]
%                             [Unstable Services, action_work]
%                         ]
%                     ]
%                     [Outside Agents Interaction Risks \S\ref{outside_agents}, action
%                         [\hphantom{x} Cooperative Complementarity Interaction Security, action
%                             [Secret Collusion Risks~\cite{motwani2023perfect}, action_work]
%                             [Amplifying Hallucination Risks~\cite{hong2023metagpt}, action_work]
%                             [Biased Decision Making Risks~\cite{pan2023risk}, action_work]
%                         ]
%                         [Competitive Interaction Security, action
%                             [Adversarial Attack Risks among Agents\cite{xu2023exploring}, action_work]
%                             [ Destructive Behavior Risks among Agents \cite{chen2023agentverse}, action_work]
%                         ]
%                     ]
                    
                
%                 ]
%         \end{forest}
%     \end{adjustbox} 
%     \caption{Typology of the interaction risk module.}
%     \label{fig:interaction}
% \end{figure*}
\begin{figure*}[tb]
\scriptsize
    \begin{adjustbox}{width=\textwidth}
        \begin{forest}
        for tree={
                forked edges,
                grow'=0,
                draw,
                rounded corners,
                node options={align=center},
                text width=2.7cm,
                s sep=6pt,
                calign=edge midpoint, 
            },
                [Interaction Security, fill=gray!45
                    [Memory Interaction Risks \S\ref{memory_interaction}, for tree={fill=gray!30}
                        [Short-term Memory Interaction Risks
                            [In-context Window Limitation Risks]
                            [Membership Inference Attack Risks~\cite{wen2023last,duan2023privacy}]
                        ]
                        [Long-term Memory Interaction Risks
                            [Poisoning Attack Risks by Indexing Processing~\cite{zou2024poisonedrag,cohen2024here}]
                            [Extracting Private Datasets Risks~\cite{zeng2024good}]
                            [RAG Generation Risks~\cite{kang2024c,hatalis2023memory}]
                        ]
                    ]
                    [API \& Tool Interaction Risks \S\ref{tool_interaction}, for tree={fill=gray!20}
                        [API Use Risks
                            [Insufficient Oversight Risks\cite{iqbal2023llm}]
                            [Authorization Risks]
                        ]
                        [API Intrinsic Risks
                            [API Security Flaws]
                            [Unstable Services]
                        ]
                    ]
                    [Outside Agents Interaction Risks \S\ref{outside_agents}, for tree={fill=gray!10}
                        [Cooperative Complementarity Interaction Security
                            [Secret Collusion Risks~\cite{motwani2023perfect}]
                            [Amplifying Hallucination Risks~\cite{hong2023metagpt}]
                            [Biased Decision Making Risks~\cite{pan2023risk}]
                        ]
                        [Competitive Interaction Security
                            [Adversarial Attack Risks among Agents~\cite{xu2023exploring}]
                            [Destructive Behavior Risks among Agents~\cite{chen2023agentverse}]
                        ]
                    ]
                ]
        \end{forest}
    \end{adjustbox} 
    \caption{Typology of the interaction risk module.}
    \label{fig:interaction}
\end{figure*}


==> figures/intro.mindmap.tex <==
% \begin{figure*}[!ht]
% \scriptsize
%     \begin{adjustbox}{width=\textwidth}
%         \begin{forest}
%         for tree={
%                 forked edges,
%                 grow'=0,
%                 draw,
%                 rounded corners,
%                 node options={align=center},
%                 text width=2.7cm,
%                 s sep=6pt,
%                 calign=edge midpoint, 
%             },
%                 [Agent Security , fill=red!45, parent
%                     [Main Agent Security \S\ref{sec:envsecurity:vir} , for tree={action} ,fill=orange!45
%                     [\hphantom{x} Prompt Template Risk,fill=orange!45, action]
%                     [LLM-based Risk,fill=orange!45,action]
%                     [Reasoning Risk,fill=orange!45,action]
%                     ]
                    
%                     [Interaction Security \S\ref{sec:envsecurity:vir} , for tree={action} ,fill=purple!45
%                     [\hphantom{x} API interaction Risks, action,fill=purple!45]
%                     [Other Agents Risks, action,fill=purple!45]
%                     ]
%                     [Environment Security \S\ref{sec:envsecurity:vir} , for tree={action} ,fill=green!45
%                     [\hphantom{x} Virtual Environment Risk, action,fill=green!45]
%                     [Physical Environment Risk, action,fill=green!45]
%                     ]
%                     [User Security \S\ref{sec:envsecurity:vir} , for tree={action},fill=blue!45
%                     [\hphantom{x} User Input Risk, action,fill=blue!45]
%                     [Malicious User Risk, action,fill=blue!45]
%                     ]
%                 ]
%         \end{forest} 
%     \end{adjustbox} 
%     \caption{Typology of (Draft version)}
%     \label{fig:sec3_mindmap_action}
% \end{figure*}

\begin{figure*}[!ht]
\scriptsize
    \begin{adjustbox}{width=\textwidth}
        \begin{forest}
        for tree={
                forked edges,
                grow'=0,
                draw,
                rounded corners,
                node options={align=center},
                text width=2.7cm,
                s sep=6pt,
                calign=edge midpoint, 
            },
                [Agent Security, fill=red!45
                    [Main Agent Security \S\ref{sec:envsecurity:vir}, for tree={fill=orange!45}
                        [Prompt Template Risk]
                        [LLM-based Risk]
                        [Reasoning Risk]
                    ]
                    [Interaction Security \S\ref{sec:envsecurity:vir}, for tree={fill=purple!45}
                        [API interaction Risks]
                        [Other Agents Risks]
                    ]
                    [Environment Security \S\ref{sec:envsecurity:vir}, for tree={fill=green!45}
                        [Virtual Environment Risk]
                        [Physical Environment Risk]
                    ]
                    [User Security \S\ref{sec:envsecurity:vir}, for tree={fill=blue!45}
                        [User Input Risk]
                        [Malicious User Risk]
                    ]
                ]
        \end{forest} 
    \end{adjustbox} 
    \caption{Typology of (Draft version)}
    \label{fig:sec3_mindmap_action}
\end{figure*}



==> figures/user_mindmap.tex <==
\begin{figure*}[!ht]
\scriptsize
    \begin{adjustbox}{width=\textwidth}
        \begin{forest}
        for tree={
                forked edges,
                grow'=0,
                draw,
                rounded corners,
                node options={align=center},
                text width=2.7cm,
                s sep=6pt,
                calign=edge midpoint, 
            },
                [User Security, fill=gray!45
                    [Unintented user input \S\ref{sec:envsecurity:vir}, for tree={fill=gray!30}
                        [Unintented feedback from human
                            [sycophancy]
                            [data breaching risk]
                        ]
                        
                        [Unintented instructions from underspecification
                        [Unsafe code execution]
                        [data breaching risk]
                        ]
                     
                    ]
                    
                    [Malicious user input\S\ref{physical_env}, for tree={fill=gray!20}
                        [Maliciously executing unsafe code risk 
                               [Detailed description needed here]
                            [Another detailed description needed here]
                        ]
                        
                        [LLM agent abuse risk
                            [Detailed description needed here]
                            [Another detailed description needed here]
                        ]

                        [Adverarial Attack Risk
                            [Detailed description needed here]
                            [Another detailed description needed here]
                        ]

                         [Jailbreak risk
                            [Detailed description needed here]
                            [Another detailed description needed here]
                        ]

                        [Inference Attacks and Contextual Learning Risk
                            [Detailed description needed here]
                            [Another detailed description needed here]
                        ]
                    ]
                ]
                
        \end{forest}
    \end{adjustbox} 
    \caption{Typology of the environment risk module.}
    \label{fig:sec3_mindmap_env}
\end{figure*}

